Comparative Performance Analysis of Intel Xeon Phi, GPU, and CPU

We investigate and characterize the performance of an important class of operations on GPUs and Many Integrated Core (MIC) architectures. Our work is motivated by applications that analyze low-dimensional spatial datasets captured by high resolution sensors, such as image datasets obtained from whole slide tissue specimens using microscopy image scanners. We identify the data access and computation patterns of operations in object segmentation and feature computation categories. We systematically implement and evaluate the performance of these core operations on modern CPUs, GPUs, and MIC systems for a microscopy image analysis application. Our results show that (1) the data access pattern and parallelization strategy employed by the operations strongly affect their performance. While the performance on a MIC of operations that perform regular data access is comparable or sometimes better than that on a GPU; (2) GPUs are significantly more efficient than MICs for operations and algorithms that irregularly access data. This is a result of the low performance of the latter when it comes to random data access; (3) adequate coordinated execution on MICs and CPUs using a performance aware task scheduling strategy improves about 1.29x over a first-come-first-served strategy. The example application attained an efficiency of 84% in an execution with of 192 nodes (3072 CPU cores and 192 MICs).

==> model.tex <==
\section{Analytical Performance Model}
\label{sec:model}
%
We present an analytical model to assess the performance of the scheduling and
optimizations proposed in this work. The main intention of this model is to
provide a set of tools to estimate the performance impact of
the proposed optimizations for a given set of tasks, which presumably comprise
a candidate application for implementation in our execution model, without
having to port the application to our system. 

The task scheduling problem in our work is dynamic in the sense that tasks may
be created during the computation, at timestamps unknown prior to the
execution. Thus, off-line scheduling is not possible and proper mapping
decisions must be carried out on-the-fly as tasks become available. The
analytical model constructed here is mostly common for all proposed scheduling
policies, which only differ in the final decision regarding to what task is
chosen for execution at each mapping time.

Let $T$ be the set of all tasks $w_i$, $1 \le i \le m$, computed by an
application during the execution, each of them created at a timestamp $c_i$ not
known prior to execution.  Assume that there is no preemption in a task
execution; each task is assigned to a single heterogeneous processor $p_j \in
p_1\dots p_n$; and, the estimated execution time of a given task $w_i$ using
processor $p_j$ is denoted as $e_{ij}$. Further, let $T^t$ be the set of tasks
created before or on timestamp $t$, which have not been scheduled for
execution.  The subset of tasks mapped to a given processor $p_j$ on or before
time $t$ is expressed as $PT_j^t$, the schedule for all processor at time $t$
as $PT^t$, and $idle_{ij}$ is the idle time elapsed between $w_i$ start time and the
end of the last task assigned to processor $p_j$.  Notice that $idle_{ij}$ may
represent several aspects as scheduling overhead, data transfer times required
to start a task, insufficient parallelism, or it could be also ignored for
simplified analysis. Further, $F(PT^t_j)$, the predicted finish time of machine
$j$ for tasks assigned on or before time $t$ may be calculated as:

\begin{equation}
F(PT^t_j) = \sum_{k \in PT_j^t} (e_{kj} + idle_{kj})
\end{equation}

In our approach, the mapping of tasks to processors is demand-driven and a
single task is assigned to a processor whenever at least one processor is
available ($\tau(PT^t) = \min_{1\le j \le n} F(PT^t_j)$), and there are tasks to be
scheduled ($T^t \neq \emptyset$). Additionally, the next non-empty set of
tasks on or after timestamp $t$ is $\zeta(t)$:

\begin{equation}
  \zeta(t) = \left\{ 
  \begin{array}{l l}
    t 		& \quad \text{if $T^t \neq \emptyset$}\\
    min_{1\le i\le m}(c_i\ |\ c_i > t) 	& \quad \text{otherwise}\\
  \end{array} \right.
\end{equation}

Thus, the next mapping time on or after a given timestamp $t$ may be calculated
as $\beta(t) = max(\tau(PT^t), \zeta(t))$. The processor to receive the next
task at a given mapping time $t'=\beta(t)$ is that processor with smallest predicted
finish time at timestamp $t'$ ($\phi(t') = \underset{1 \le j \le
n}{\operatorname{argmin}}\ F(PT^{t'}_j)$). Further, we define the function
$\vartheta(t)$ that calculates the mapping of a single task at time $t$:

\begin{equation}
\vartheta(t) = \beta(\tau(PT_{\phi(t)}^t \leftarrow select(T^{t}, POLICY)))
\label{eq:mapping}
\end{equation}

%\begin{equation}
%\vartheta(t) = \beta(\tau(PT_{\phi(\beta(t))} \leftarrow select(T^{\beta(t)}, POLICY)))
%\label{eq:mapping}
%\end{equation}

The $\vartheta(t)$ first calculates the set of tasks ready to execute at the
mapping time $t$ ($T^{t}$), selects one task according to the scheduling policy
chosen, e.g. FCFS or PRIORITY, and assigns that task to the processor with
minimum finish time at time $t$ ($\phi(t)$). After the mapping is performed, the
timestamp of the next mapping is computed as a result.

In practice, the overall schedule is calculated as a sequence of $m$ mappings,
which are dynamically calculated based on the previous mappings results. Thus,
the global schedule may computed recursively using function $Z(m)$ that
utilizes $\vartheta(t)$ defined before to compute every single mapping.  As
shown bellow, the result of each $Z(N)$ is the timestamp of the next
mapping ($N + 1$), which is recursively given as input to $\vartheta(t)$.

\begin{equation}
  Z(m) = \left\{ 
  \begin{array}{l l}
    \beta(0) 		& \quad \text{if $ m = 0$}\\
    \vartheta(Z(m-1))	& \quad \text{otherwise}\\
  \end{array} \right.
%\vartheta(N) = PT_{\phi(\beta(t))} \leftarrow select(T^{\beta(t)}), t'=\beta(t)
\label{eq:mapping2}
\end{equation}

After $m$ mappings, the makespan may be calculated as the $max_{1\le j \le n}
F_j(Z(m))$, or optionally as $max_{1\le j \le n} F_j(\infty)$.  The performance
of the scheduling policies in this framework are differentiated through the
$select$ function implemented by each of them. While FCFS chooses the task with
smallest creation time $c_i \in T^{\beta(t)}$, PRIORITY orders the task in
$T^{\beta(t)}$ according to the expected speedup to select that task with
highest speedups to the GPU and smallest speedup to the CPU. 

